Scalar curvature in conformal geometry of Connes-Landi noncommutative manifolds

We first propose a conformal geometry for Connes-Landi noncommutative manifolds and study the associated scalar curvature. The new scalar curvature contains its Riemannian counterpart as the commutative limit. Similar to the results on noncommutative two tori, the quantum part of the curvature consists of actions of the modular derivation through two local curvature functions. Explicit expressions for those functions are obtained for all even dimensions (greater than two). In dimension four, the one variable function shows striking similarity to the analytic functions of the characteristic classes appeared in the Atiyah-Singer local index formula, namely, it is roughly a product of the $j$-function (which defines the $\hat A$-class of a manifold) and an exponential function (which defines the Chern character of a bundle). By performing two different computations for the variation of the Einstein-Hilbert action, we obtain a deep internal relations between two local curvature functions. Straightforward verification for those relations gives a strong conceptual confirmation for the whole computational machinery we have developed so far, especially the Mathematica code hidden behind the paper.

==> introv2.tex <==
\section{Introduction}

The origin of noncommutative geometry started by Alain Connes in the 80's was heavily influenced by the two pillars in twentieth century physics: Einstein's GR (general relativity) and quantum physics with  Heisenberg's formulation of matrix mechanics.  Einstein's GR is a geometrization  of the theory of gravitation based on Riemann's paradigm of geometry. Quote from Connes' essay \cite{MR1826266}: 
\begin{quotation}
 On reflection, this discovery actually clearly displays the limitation of Riemann's formulation of geometry. If we look at the phase space of an atomic system and follow Riemann's procedure to parametrize its points by finitely many real numbers, $\dots$  However, according to Heisenberg this doesn't work because as soon as we make the first measurement, we alter the situation drastically.  $\dots$ The starting point of noncommutative geometry is to take this new notion of space seriously.    
\end{quotation}

In physics, the idea that the spacetime coordinates do not commute goes back to 1947 \cite{MR0019438}. A profound achievement in  Connes's noncommutative geometry is an extension of  the notion of metric, from ordinary manifolds to a new class of noncommutative space in the frame work of functional analysis (to be more precise, the theory of operator algebras). A significant point is that such extension contains Riemannian geometry as a special
case\footnote{In fact, more properties for such an extension are expected from physics point of view, see \cite[Ch.1, Sec.10]{connes2008noncommutative} }. \par

For a $C^*$-algebra $A$ (not necessary commutative), viewed as coordinate algebra of certain noncommutative space, a metric structure is given by a spectral triple $(\mathcal A, \mathcal H, D)$. The algebra $\mathcal A \subset A$ is a dense, holomorphically closed subalgebra with a representation  $\mathcal A \subset B(\mathcal H)$ as bounded operators on the Hilbert space $\mathcal H$. The metric structure is brought in via the unbounded, self-adjoint operator $D$ on $\mathcal H$
(playing the role of the Dirac operator) with the bounded commutator property, namely $\forall a \in \mathcal A$, the commutator $[D,a] = D a -a D$ are well-defined and bounded. The prototypical example comes from Connes's Dirac model for spin geometry: $(C^\infty(M), L^2(\slashed S), \slashed D)$, where $M$ is a closed spin manifold with  spinor bundle $\slashed S$ and the associated Dirac operator $\slashed D$. Any introduction level  books and essays in noncommutative will
given a quick  comparison between the spectral notions and the classical
notions in spin geometry, here we only list Connes's book \cite{MR1303779} as a starting point. The geometry derived from the spectral setting is still growing rapidly. In the lecture note \cite{MR2408150}, twenty-four examples distributed  among geometry-topology, number theory and  mathematical physics are discussed. Those are the prominent applications of the global aspect of noncommutative geometry. \par
% In contrast, the local aspect of noncommutative geometry, such as the concept of intrinsic curvature, has recently (2014) begun to be comprehended in the development of modular geometry on noncommutative two/four tori.       

% So far, we have included the notion of Riemannian metric in our spectral frame work, what is the next essential concept in Riemannian geometry? The answer is concept of intrinsic curvature, whose description relies  heavily on local charts which is the first thing we have to give up when passing to the noncommutative world. In the spectral setting, the notation of local invariants like intrinsic curvature are much less transparent, they can only been seen through  
In contrast, the local aspect of has only recently begun to be understand by the local geometry on the simplest noncommutative Riemann surface: noncommutative two tori developed in Connes-Moscovici  \cite{MR3194491} around 2014. In this paper, we study the local geometry for a class of noncommutative manifold $(C^\infty(M_\theta), L^2(\slashed S), \slashed D)$, where $\theta$ is a skew symmetric matrix, obtained by deforming the Dirac model spectral triples along a torus action introduced by Connes-Landi in \cite{MR1846904}. They are
sometimes called almost commutative manifolds. Nevertheless, after introducing a family of noncommutative metrics, the local geometry becomes high nontrivial. To pass to the noncommutative setting, we start with some central results in the spectral geometry of Riemannian manifolds. \par   

In Riemannian geometry,  the next essential notion after metric is the concept of intrinsic curvature, whose description relies  heavily on local charts which is the first thing we have to give up when passing to the noncommutative world. In the spectral setting, the notations of local invariants like intrinsic curvature still exist, but are much less transparent. They can only been seen through spectral functionals related to the high frequency behavior of the spectrum of $D$ in the
spectral triple coupled with the action of the algebra of coordinates $\mathcal A$.  The motivation comes from the spectral geometry of  closed Riemannian manifolds. For the  consistency of our discussion, let us assume that the manifold $M$ is spin with a Dirac model spectral triple $(C^\infty(M), L^2(\slashed S), \slashed D)$. The heat kernel asymptotic plays the central role in the spectrum geometry: 
\begin{align}
    e^{-t\slashed D^2}(t,x,x) \backsim_{t \searrow 0} \sum_{j=0}^\infty V_j(x,\slashed D^2) t^{(j-m)/2}, \,\,\, x \in M, \,\, m=\dim M.
    \label{eq:intro-heatkernel-asym}
\end{align}
All $V_j(x,\slashed D^2)$ are smooth sections valued in $\End(\slashed S)$. In local charts, they can be written as polynomials whose arguments consist of all the components of the Riemannian curvature tensor, the curvature tensor on the spinor bundle and  their covariant derivatives. The pioneers are Hadamard, Minakshisundaram-Pleijel, Seeley-De Witt.  The standard reference for the topics mentioned above is Gilkey's book \cite{gilkey1995invariance}. \par
The operator-theoretical version of \eqref{eq:intro-heatkernel-asym} is the trace functional $\Tr(f e^{-tD^2})$: 
$\forall f\in C^\infty(M),$
\begin{align}
    \Tr(f e^{-tD^2}) \backsim_{t \searrow 0} \sum_{j=0}^\infty V_j(f,D^2) t^{(j-m)/2}, \,\, \,
    \,\,\, m=\dim M.
    \label{eq:intro-heatasym}
\end{align}
Each coefficient $V_j(f,D^2)$ is an example of ``spectral  functional'' (in $f$) mentioned before. The two version are equivalent in the following sense: $V_j(x,D^2)$ are the functional densities of $V_j(f,D^2)$ with respect to the tracial functional $\varphi_0$.
  To be precise, 
 \begin{align*}
    V_j(f,D^2) = \varphi_0(f V_j(x,D^2)) , \,\,\, \forall f\in C^\infty(M),
\end{align*}
here $\varphi_0(\psi) = \int_M \Tr_x(\psi) \mathrm d\op{vol}_g$, $\forall \psi \in \Gamma(\End(\slashed S))$, where $\Tr_x$ is the fiberwise trace. \par

What is important for us is the subleading term of the expansion, that is the case with $j=2$. Apply the general results in Gilkey's book \cite{gilkey1995invariance} to the squared of the spinor Dirac $\slashed D$, we have: upto an overall constant $(4\pi)^{-m/2}$, $V_0(x,\slashed D^2) = I$ which is related to the volume form and the next term recovers the scalar curvature function $\mathcal S_{\slashed D}$:
\begin{align}
    V_2(x,\slashed D^2) = \frac{-1}{12} \mathcal S_{\slashed D}. 
    \label{eq:intro-V2term-local}
\end{align}
This result leads to our Definition \ref{defn:scalcur-RDh} of the scalar curvature for our noncommutative manifolds. More Definition \ref{defn:scalcur-RDh} can be restated as Definition 1.147 in  Connes-Marcolli's book \cite{connes2008noncommutative} in a intrinsic fashion\footnote{However, such intrinsic formulation does not help the computation, thus we remind the readers the fact to emphasize the point that our scalar curvature depends only on the data given in  spectral triples.}.  One
can also find more detailed discussion for the computation of  \eqref{eq:intro-V2term-local} in the same book, in the proof of Theorem 11.1. 
\par


% 
% the spectral function $V_2(\cdot,D^2)$ recovers the notion of scalar curvature (see \eqref{eq:intro-V2term-local}). \par
% For instance,  in particular, for \eqref{eq:intro-V2term-local}, 
% 

We can push the discussion further to introduce a family of noncommutative metrics using our spectral framework. Back to Riemannian geometry, we often consider a family of metrics $(M,g_\varepsilon)$ on a manifold parametrized by $\varepsilon>0$ and study the related variation problems. Use the spectral language, $(M,g_\varepsilon)$ gives rise to  a family of spectral triples $(C^\infty(M), L^2(\slashed S_{g_\varepsilon}), \slashed D_{g_\varepsilon})$. From functional analytic
perspective, the all the separable Hilbert are identical, therefore one can fix the  Hilbert space, say the one with $\varepsilon =0$, so that all the operators have a common domain, which is crucial for studying the variation problems. The price to pay is that we have to deal with a family of perturbed Dirac operators. They do not even satisfy the bounded commutator axiom of the spectral triple. This fact  dramatically increases the complexity of the computation. In spin geometry, this  idea
was pursued  in \cite{MR1158762}, the result is the following: for each $\varepsilon$, there exists a canonical gauge transformation $\beta^{g_0}_{g_\varepsilon}$  sending  $g_\varepsilon$-spinor sections to $g_0$-spinor sections. The associated gauge transformed Dirac operators were computed explicitly in \cite{MR1158762} as well. In order to get a unitary operator $U_\varepsilon: L^2(\slashed
S_{g_\varepsilon}) \rightarrow L^2(\slashed S_{g_0})$ at the level of $L^2$-sections, one needs to 
add the change of volume form to the gauge transformation. Finally the perturbed Dirac operator looks like: $D_\varepsilon =U_\varepsilon \circ \slashed D_{g_\varepsilon} \circ U^{-1}_\varepsilon$. In this paper, we only study the conformal change of metric $g' = e^{2h} g$, where $h$ is a real-valued smooth function, the perturbation of the  Dirac operator is given by $D_h = e^{h/2} \slashed D e^{h/2}$. See Section \ref{sec:scalcur-con-ch-met} for more details. 

\par
In the noncommutative setting, one should simply take the perturbed Dirac operators $D_\varepsilon$ as a starting point to represent a family of metrics. For instance, consider the Connes-Landi deformation spectral triple $(C^\infty(M_\theta), L^2(\slashed S),\slashed D)$, here the spinor Dirac $\slashed D$ represents the underlying Riemannian metric $g$. The conformal class of metrics with respect to $g$ on the spectral triple consists of all the gauge transformed Dirac operators of the form $D_h = e^{h/2}
\slashed D e^{h/2}$, where $h = h^* \in C^\infty(M_\theta)$ can be any self-adjoint elements in the coordinate algebra. The associated  scalar curvature $R_{ D_h} \in C^\infty(M_\theta)$ (Definition \ref{defn:scalcur-RDh}) is the local expression of the functional $V_2(\cdot, D^2_h)$ in \eqref{eq:intro-heatasym}. 
\par

Our first main result is the explicit formula for the curvature: 
\begin{align}
            \label{eq:intro-RDlogk}
        R_{ D_h} &= \, e^{(-m+2)h} \brac{
            \mathcal K^{(m)}_{\slashed D_h}(\logmodop) (\nabla^2 h) + 
    \mathcal H^{(m)}_{\slashed D_h}(\logmodop_{(1)}, \logmodop_{(2)})(\nabla h \nabla h)
} g^{-1}  \\
&+c_{\Delta_k} e^{(-m+2)h} \mathcal S_\Delta , \,\,\,\nonumber
    \end{align}
where $m=\dim M \ge 4$ is  even. 

For the deformed spectral triple, we do not even have a family of spectral triples to start. However, this makes our lives easier, we simply fix the algebra and the Hilbert space, while the family of noncommutative metric are represented by the family of
perturbed Dirac operators $D_\varepsilon$, and then the associated scalar curvature is given by the functional density of $V_2(\cdot, D^2_\varepsilon)$ in the heat asymptotic \eqref{eq:intro-heatasym}. In \cite{MR3194491}, the curved geometry for noncommutative two tori was constructed in a different way, but what is in common is that we both want to  fix a Hilbert space and perturbed the Dirac operator and its adjoint (if necessary). The price to pay is hidden in the computation side.
After perturbation, namely when $\varepsilon \neq 0$, we have left out comfort zone: spectral triples, for instance, the commutators $[D_\varepsilon, f]$, where $f$ is a coordinate function, fail to be bounded operators. Many tools in the global aspect do not apply to the local side. The essential technical tools used for local computation are pseudo differential calculi. On noncommutative tori without coefficients, the calculus was developed in Connes's seminar paper: \cite{connes1980c}.
An upgraded version in which  the coefficients are Heisenberg modules was explained in \cite{MR3540454}. For Connes-Landi deformations, the construction of a pseudo differential calculus which is suitable for studying the spectral geometry is one of the mains results in the authors previous work \cite{Liu:2015dfa}. \par

We are ready to state our main results. Let $(C^\infty(M_\theta), L^2(\slashed S),\slashed D)$ be a Connes-Landi deformation spectral triple, in which the algebra $C^\infty(M_\theta) \defeq (C^\infty(M),\times_\theta)$ is identical to $C^\infty(M)$ as a topological vector equipped with a new family of multiplications parametrized by skew symmetric matrices $\theta$. In order to perform the deformation, we required that the group $\op{Iso}(M)$ of isometries of $M$ contains a
$n$-torus, also $M$ should be spin so that the spinor bundle $\slashed S$ and the spinor Dirac operator $\slashed D$ make sense. Thanks to the functorial property of the deformation (cf. \cite{MR3262521}), $C^\infty(M)$-modules like spinor sections $\Gamma(\slashed S)$, differential forms $\Gamma(T^*M)$ and vector fields $\Gamma(TM)$ become $C^\infty(M_\theta)$-bimodules (the left and right actions are different now). In particular, we have $C^\infty(M_\theta) \subset
B(L^2(\slashed S))$ via deformed left action. The Dirac operator $\slashed D$ stays the same during the deformation which gives rise to a spectral triple mention before as a standard (commutative) metric for the underlying commutative manifold. The family of noncommutative metrics considered in this paper is the class of conformal metrics with respect to the starting metric $\slashed D$. In Riemannian geometry, a conformal metric is given by $g' = e^{2h} g$, where $h$ is a real-valued
smooth function on the manifold. The function $e^h$ is called a Weyl factor\footnote{The name comes from physics side, in which conformal transformations are often called Weyl transformations.} or a conformal factor. The gauge transformed Dirac operator is of the form $D_h = e^{h/2}\slashed D e^{h/2}$ (see Section. \ref{sec:scalcur-con-ch-met}). In the noncommutative setting, The conformal change of metric is defined to be  the family of  perturbed Dirac operator $D_h =
e^{h/2}\slashed D e^{h/2}$, in which the real valued function becomes a self-adjoint operator $h = h^* \in C^\infty(M_\theta)$ and  the Weyl factor $e^h$ is defined with respect to the deformed multiplication.  
    
% \begin{align*}
%     \varphi_0(\psi) = \int_M \Tr_x(\psi) \mathrm d\op{vol}_g, 
% \end{align*}
% 
%it depends on $f$ and the asymptotic behavior of the spectrum of $\slashed D$ at infinity. However  



This idea was deeply implemented on the simplest noncommutative Riemann surface: noncommutative two tori. The early calculation for this program is the Gauss-Bonnet theorem for noncommutative two tori Connes-Tretkoff \cite{MR2907006}. The full computation of the scalar curvature and the modular geometry was developed in Connes-Moscovici  \cite{MR3194491}. The assistant from CAS (computer algebra
system)\footnote{\textsf{Mathematica} was used in \cite{MR2907006} and \cite{MR3194491}.} plays a
role involved in both paper. Another team Khalkhali-Fathizadeh  performed the same computation (for the Gauss-Bonnet theorem and the full expression for the curvature) independently in \cite{MR2956317} and \cite{MR3148618} using a different CAS. Later they studied the modular geometry for noncommutative four tori in \cite{MR3359018} and \cite{MR3369894}. In \cite{leschdivideddifference}, Lesch gave some deep conceptual understanding about  the local curvature functions appeared in
\cite{MR3194491} and gave a different proof for the rearmament lemma with a firm functional analytic ground. Another important progress made by Lesch-Moscovici \cite{MR3540454} is to extend the Ray-Singer log-determinant functional to Heisenberg bimodules over pairs of Morita equivalent noncommutative tori. A novel discovery is that the scalar curvature has certain Morita invariance property which is a purely noncommutative phenomenon. On noncommutative two tori, there are some different
approaches: see \cite{Bhuyain2012}  and \cite{2013SIGMA...9..071R}. Some new progress on noncommutative tori \cite{2014arXiv1410.0475F} and \cite{2016arXiv161004740K}.
\par

In this paper, we study a larger class of noncommutative manifolds known as Connes-Landi deformation. The spectral triple of such noncommutative space was first proposed in   Connes-Landi \cite{MR1846904} and then further refined in Connes and Dubois-Violette, \cite{MR1937657} and \cite{MR2403605}. The analytic aspect of the deformation theory (known as $\theta$-deformation) was developed even earlier by Rieffel \cite{MR1184061}. The reason the author started to look at those
examples is the gauge theory aspects studied in Brain-Landi-van Suijlekom \cite{MR3262521}. Other work related to the analytic aspect of the deformation is  Gayral-Iochum-V\'arilly \cite{MR2230348}.





















